Universal Vassiliev invariants of links in coverings of 3-manifolds

We study Vassiliev invariants of links in a 3-manifold $M$ by using chord diagrams labeled by elements of the fundamental group of $M$. We construct universal Vassiliev invariants of links in $M$, where $M=P^2\times [0,1]$ is a cylinder over the real projective plane $P^2$, $M=\Sigma\times [0,1]$ is a cylinder over a surface $\Sigma$ with boundary, and $M=S^1\times S^2$. A finite covering $p:N\longrightarrow M$ induces a map $\pi_1(p)^*$ between labeled chord diagrams that corresponds to taking the preimage $p^{-1}(L)\subset N$ of a link $L\subset M$. The maps $p^{-1}$ and $\pi_1(p)^*$ intertwine the constructed universal Vassiliev invariants.

==> fig/Abar.tex <==
\begin{picture}(0,0)%
\epsfig{file=Abar.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(519,402)(1039,-711)
\end{picture}


==> fig/Bbar.tex <==
\begin{picture}(0,0)%
\epsfig{file=Bbar.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(519,402)(1594,-711)
\end{picture}


==> fig/X.tex <==
\begin{picture}(0,0)%
\epsfig{file=X.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(229,192)(2314,-2275)
\end{picture}


==> fig/cchords.tex <==
\begin{picture}(0,0)%
\epsfig{file=cchords.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(424,244)(1939,-558)
\end{picture}


==> fig/chord.tex <==
\begin{picture}(0,0)%
\includegraphics{chord.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(344,344)(1179,-683)
\end{picture}


==> fig/dop.tex <==
\begin{picture}(0,0)%
\epsfig{file=dop.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(359,344)(1529,-46)
\end{picture}


==> fig/m1.tex <==
\begin{picture}(0,0)%
\epsfig{file=m1.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4201,1119)(1789,-584)
\put(3790,-234){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\leftrightsquigarrow$}}}
\end{picture}


==> fig/m2.tex <==
\begin{picture}(0,0)%
\epsfig{file=m2.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4485,924)(2792,-695)
\put(4925,-392){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\leftrightsquigarrow$}}}
\end{picture}


==> fig/m3.tex <==
\begin{picture}(0,0)%
\epsfig{file=m3.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4402,1228)(2879,-690)
\put(4939,-311){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\leftrightsquigarrow$}}}
\end{picture}


==> fig/m4.tex <==
\begin{picture}(0,0)%
\epsfig{file=m4.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4555,972)(2733,-709)
\put(4955,-404){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\leftrightsquigarrow$}}}
\end{picture}


==> fig/rp2fi.tex <==
\begin{picture}(0,0)%
\epsfig{file=rp2fi.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4449,1936)(964,-2248)
\put(3076,-1636){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\leftrightsquigarrow$}}}
\end{picture}


==> fig/stdpos.tex <==
\begin{picture}(0,0)%
\epsfig{file=stdpos.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1244,624)(1179,-973)
\put(1351,-736){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\vdots$}}}
\put(2176,-736){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}$\vdots$}}}
\end{picture}


==> wks/wks11.tex <==
\section{An analogue of the Conway polynomial}\label{s:C}

The link invariant $Z_{\Sigma\times I}$ of Lemma~\ref{l:Kontsevi} is 
interesting for theoretical reasons because it allows to prove the
isomorphism ${\cal V}(\Sigma\times I)\cong\Ab(\Sigma\times I)^*$,
but even in low degrees 
it takes much time to calculace~$Z_{\Sigma\times I}(L)$ for a link~$L$.
Therefore we study in the following sections
specializations of~$Z_{\Sigma\times I}$ that are
simpler to evaluate.

For a set $X$, let $V_X$ be the vector space with
basis~$\{t_x\,\vert\, x\in X\}$.
Let $G$ be a group and let $\sigma:G\longrightarrow \{\pm 1\}$ be a
homomorphism of groups. Define $\sigmab:G\longrightarrow\Z/(2)$ by
$\sigma(g)=(-1)^{\sigmab(g)}$.
Let $I_G^\sigma$ be the ideal in the tensor algebra
${\cal T}(V_G)$ of $V_G$ generated by the
elements $t_{gh}-(-1)^{\sigmab(g)\sigmab(h)}t_{hg}$
and~$t_gt_h-(-1)^{\sigmab(g)\sigmab(h)}t_ht_g$. We define
$\oQGs={\cal T}(V_G)/I_G^\sigma$.
Assume that we have chosen a set $\Conj$ of
representatives of conjugacy classes of elements of $G$. Let

\begin{equation}
\Conj(\bar{0})=\left\{a\in \Conj\,\vert\, 
\sigmab(a)=\bar{0}\mbox{ and }
N_a\subseteq\Ker\,\sigma\right\},
\end{equation}

where $N_a=\{b\,\vert\, ab=ba\}$ is the normalizer of~$a$. 
Let $\Conj(\bar{1})=\Conj\cap \sigmab^{-1}(\bar{1})$. Then
it is easy to see that we have an isomorphism of algebras

\begin{equation}\label{e:RGsiso}
\oQGs\cong S\left(V_{\Conj(\bar{0})}\right)\otimes
\Lambda\left(V_{\Conj(\bar{1})}\right),
\end{equation}

where $S(V)$ denotes the symmetric algebra and $\Lambda(V)$ denotes
the antisymmetric algebra of a vector space~$V$. Let

\begin{equation}
\RbGs=\left\{
\begin{array}{ll}
R(G,\sigma)/(t_e^2) & \mbox{if $G=\{e\}$,}\\
R(G,\sigma)/(t_e) & \mbox{otherwise.}
\end{array}
\right.
\end{equation}

For $\sigma\not=1$ we have $R(G,\sigma)=\RbGs$.

Let $\Sigma$ be a connected compact surface.
If~$\Sigma$ has non-empty boundary, then we choose a decomposition
$(B_\nu,J_\mu)$ of~$\Sigma$ as in Definition~\ref{d:decsu}.
If~$\Sigma$ has empty boundary, then we choose~$B\subset \Sigma$ with
$B\cong D^2$, and a decomposition of $\Sigma\setminus B^\circ$.
The rest of this section will depend on these choices.

Let~$*\in B_0\times I$. 
We choose a linearly ordered 
set~$(\Conj,\leq)$ of representatives of conjugacy classes
in~$\pi_1(\Sigma\times I,*)$. We can do this for example in the
following way.
Choose generators $a_1,\ldots,a_k$ of $\pi_1(\Sigma\times I,*)$, where
$a_i$ passes one time through the band $B_i$ in the
counterclockwise sense in our pictures.
We define a linear order on words~$r,r'\ldots$ in the
alphabet $a_1,a_1^{-1},a_2,\ldots,a_k^{-1}$ as follows: we say that
$r\leq r'$ if $l(r)< l(r')$ or $l(r)=l(r')$ and $r\leq_\lex r'$, where
$l(r)\in\N$ denotes the length of the word~$r$ and $\leq_\lex$ denotes
the lexicographic order. We define an order on $\pi_1(\Sigma\times I,*)$ by
using minimal expressions in the generators~$a_i$.
Let $\Conj$ be the set of representatives of conjugacy classes given by
the elements that are minimal in their conjugacy class.
The order on $\pi_1(\Sigma\times I,*)$ induces an order on~$\Conj$.
As in Section~\ref{s:psi} we identify elements of $\pi_1(\Sigma\times
I,*)$ with homotopy classes of paths between points in~$B_0\times I$.

\begin{defi}
We call the projection from $\Sigma\times I$ to $I$ the height.
A link $L\subset \Sigma\times I$ is called {\em descending}, if it has
the following properties:

(a) Let~$K$ be a component of $L$. Then a highest point $p$ of $K$ lies
inside~$B_0\times I$.
If we travel along $K$ starting at $p$, then the height descends
strictly and we follow a path $g\in \Conj$. Arriving at the lowest point
of~$K$ one returns to the
height of~$p$ very close to  
$J_1 \times I$.

(b) The projections of the components of $L$ to $I$ are disjoint.
Then the orientation of~$I$ induces an order $K_1,\ldots,K_m$ on the
components of $L$. Let $g_\nu\in \Conj$ be the element
belonging to the component $K_\nu$. Then we have $g_1\geq\ldots\geq g_m$.
\end{defi}

For diagrams of a descending link we can rephrase Condition~(a) of the
definition as follows: If we start at a point $p$ of a component~$K$ 
lying very close
to $J_1$ and travel along $K$, then we follow a path $g\in \Conj$ and
traverse each crossing between strands of~$K$
first at the overcrossing strand.


Now let~$G=\pi_1(\Sigma\times I,*)$ and let
$\sigma:G\longrightarrow\{\pm 1\}$ be defined as in Section~\ref{singlink}.
Let

\begin{equation}
R(\Sigma)=R(\pi_1(\Sigma\times I),\sigma)\quad\mbox{and}\quad
\RbS=\Rb(\pi_1(\Sigma\times I,*),\sigma).
\end{equation}

A based link $L\subset\Sigma\times I$ is a link with
a chosen basepoint on each component of~$L$
inside $B_0 \times I$. We do not allow a basepoint to leave
$B_0\times I$ during an isotopy.
An ordered based link is a based link with a linear order of its components.
For an ordered based link~$L$ we define the
monomial~$t_L\in {\cal T}(V_G)$
as the ordered product over all components~$K$ of~$L$ of the
elements~$t_g$, where~$K$
with the basepoint as starting point is
a representative of~$g\in\pi_1(\Sigma\times I,*)$.
We also denote the image of~$t_L$ in~$R(\Sigma)$ and
in~$\RbS$ by~$t_L$.
A monomial $t_{g_1}\ldots t_{g_k}$ is called standard if~$g_\nu\in C$
and if $g_1\leq\ldots\leq g_k$. 
We define the linear map
$\theta:R(\Sigma)\longrightarrow\Q$ by specifying the values of
standard monomials as

\begin{equation}\label{e:deftheta}
\theta(t_{g_1}\ldots t_{g_k})=\left\{
\begin{array}{ll}
 0 & \mbox{if $t_{g_1}\ldots t_{g_k}=0\in R(\Sigma)$,}\\
 1 & \mbox{otherwise.}
\end{array}
\right.
\end{equation}

Let~$L$ be a singular ordered based link with one double point.
We assume that the double point of $L$ lies inside $B_0\times I$.
The singular link~$L$ is the image of~$\ell$ ordered based
circles. We draw the circles in increasing order.
We connect the two points on these circles that are the preimages of
the double point of~$L$ by a chord.
We label this chord diagram by
elements of $\pi_1(\Sigma\times I,*)$ as shown in Figure~\ref{f:double1} and
Figure~\ref{f:double2} for the two possible cases, where
the label on an interval between basepoints or chord endpoints on the
circles is represented by the image of this interval in~$\Sigma\times I$.
Denote the resulting \labelled{} chord diagram equipped with the basepoints
and with the order on its components by~$D_L$.

\begin{figure}[!h]
\centering
\vcentre{onechord1}
\caption{The chord lies on one circle}\label{f:double1}
\end{figure}

\begin{figure}[!h]
\centering
\vcentre{onechord2}
\caption{The chord connects two circles}\label{f:double2}
\end{figure}

We define $\gamma(L)\in\{\pm 1\}$ and $\gamma(D_L)\in\{\pm 1\}$ by

\begin{equation}\label{e:defgamma}
\gamma(L)=\gamma(D_L)=\left\{
\begin{array}{ll}
(-1)^{\bar{\sigma}(b)\bar{\sigma}(c)} &
\mbox{in the case of Figure~\ref{f:double1},}\\
(-1)^{\bar{\sigma}(c)\bar{\sigma}(d)+\bar{\sigma}(cd)
\bar{\sigma}(bg_m\ldots g_n)} & \mbox{in the case of
Figure~\ref{f:double2}.}
\end{array}
\right.
\end{equation}

We say that ordered based links $(L_+,L_-,L_{\vert\vert})$
form a {\em skein triple}, if they have the following properties.

\begin{itemize}
\item They differ inside of a ball
$D^3\subset B_0\times I$ as the diagrams
$L_+,L_-,L_{\vert\vert}$ of Figure~\ref{f:hkpict} and coincide on the
outside of this ball.

\item The order and the basepoints of the components of $L_+$ and $L_-$
are the same.

\item Let $L_\times$ be the singular ordered based link of 
Figure~\ref{f:hkpict} with one double point.
Then the relation between the basepoints and the
order of the components of~$L_{\vert\vert}$ and the basepoints and the
order of the components of~$L_+$ and~$L_-$ is illustrated in
Figures~\ref{f:ord1} and~\ref{f:ord2} for the two possible cases of
Figures~\ref{f:double1} and~\ref{f:double2}.
\end{itemize}

\begin{figure}[!h]
$$
\Picture{
\thicklines
\put(1,1){\vector(-1,-1){2}}
\put(-1,1){\vector(1,-1){2}}
\put(-1,-1.8){\makebox(2,0.7){$L_\times$}}
}
\qquad
\Picture{
\thicklines
\put(1,1){\vector(-1,-1){2}}
\put(-1,1){\line(1,-1){0.83}}
\put(0.17,-0.17){\vector(1,-1){0.83}}
\put(-1,-1.8){\makebox(2,0.7){$L_+$}}
}
\qquad
\Picture{
\thicklines
\put(1,1){\line(-1,-1){0.83}}
\put(-0.17,-0.17){\vector(-1,-1){0.83}}
\put(-1,1){\vector(1,-1){2}}
\put(-1,-1.8){\makebox(2,0.7){$L_-$}}
}
\qquad
\Picture{
\thicklines
\qbezier[90](1,1)(0,0)(1,-1)
\qbezier[90](-1,1)(0,0)(-1,-1)
\put(-0.9,-0.9){\vector(-1,-1){0.1}}
\put(0.9,-0.9){\vector(1,-1){0.1}}
\put(-1,-1.8){\makebox(2,0.7){$L_{\mid\mid}$}}
}
\qquad
\Picture{
\thicklines
\qbezier[90](1,1)(0,0)(-1,1)
\qbezier[90](1,-1)(0,0)(-1,-1)
\put(-1,-1.8){\makebox(2,0.7){$L_=$}}
}
$$\nopagebreak\vspace*{15pt}
\caption{Local modifications of a link}\label{f:hkpict}
\end{figure}

\begin{figure}[!h]
\centering
\vcentre{nochord1}
\caption{A new order in the first case}\label{f:ord1}
\end{figure}

\begin{figure}[!h]
\centering
\vcentre{nochord2}
\caption{A new order in the second case}\label{f:ord2}
\end{figure}

The property of an ordered based link to be descending is unrelated to
the order of its components and is also unrelated to the basepoints.

\begin{theorem}\label{t:C}
(1) Let~$\Sigma$ be a connected compact surface with non-empty
boundary or let~$\Sigma$ be the real projective plane.
Then
there exists a unique isotopy invariant
$C^\ob(L)\in \Ring(\Sigma\times I)[z]$ of ordered
based links~$L$ in $\Sigma\times I$ having the following properties:

\begin{eqnarray}
& & C^\ob(L_+)-C^\ob(L_-) =
\gamma(L_\times) z C^\ob(L_{\mid\mid}), 
\label{skeinC}\\
& & C^\ob(L)=t_L,\ \mbox{if $L$ is descending,}\label{e:Cdesc}
\end{eqnarray}

where Equation~(\ref{skeinC}) holds for all skein triples
$(L_+,L_-,L_{\mid\mid})$.

(2) If $L$ is a link in $\Sigma\times I$,
then we turn~$L$ in an arbitrary way into an ordered
based link~$L'$.
Then the formula~$C(L)=\theta(t_{L'}) C^\ob(L')$
defines an isotopy invariant of~$L$.
\end{theorem}

Theorem~\ref{t:C} shall be proved in Section~\ref{s:eC}.
We call the link invariant~$C$ the {\em Conway} polynomial.
Equations~(\ref{skeinC}) and~(\ref{e:Cdesc}) are sufficient to
calculate~$C^\ob(L)$ for every ordered based link~$L$.
Let~$\tilde{C}$ be the usual Conway polynomial of links 
in~$I^2\times I$ (\cite{Con}). 
We have~$\Rb(I^2)\cong \Q\oplus\Q t_e$ as a vector space and the
sign~$\gamma(L_\times)$ is always~$1$. This implies
$C(L)=\tilde{C}(L)t_e$ for any link~$L\subset I^2\times I$
because this equation holds for descending links and the
polynomials~$C$ and~$\tilde{C}$ satisfy the same equation on each
triple $(L_+,L_-,L_{\vert\vert})$ of links 
that differ as shown in Figure~\ref{f:hkpict}.
%If~$\Sigma$ is orientable, then $C$ is a specialization of the Homfly
%polynomial of links in $\Sigma\times I$.
Let us consider a further example. 
Let~$L$ be a link in~$P^2\times I$ and let~$L'$ be a link
in~$I^2\times I$ 
as in Figure~\ref{f:Conway}, where the parts of the link diagrams
consisting of a box \labelled{}~$T$ are identical.

\begin{figure}[!h]
\centering
\vcentre{cex}
\caption{A link in $P^2\times I$ and a link in $I^2\times I$}
\label{f:Conway}
\end{figure}

Then we have 

\begin{equation}
C(L)=\left\{
\begin{array}{ll}
\tilde{C}(L')t_u & \mbox{if $L$ is a knot,}\\
0 & \mbox{otherwise,}
\end{array}
\right.
\end{equation}

where~$u$ denotes the unique non-trivial
element of $\pi_1(P^2\times I,*)$.


